Trusted Confidence Bounds for Learning Enabled Cyber-Physical Systems

Cyber-physical systems (CPS) can benefit by the use of learning enabled components (LECs) such as deep neural networks (DNNs) for perception and decision making tasks. However, DNNs are typically non-transparent making reasoning about their predictions very difficult, and hence their application to safety-critical systems is very challenging. LECs could be integrated easier into CPS if their predictions could be complemented with a confidence measure that quantifies how much we trust their output. The paper presents an approach for computing confidence bounds based on Inductive Conformal Prediction (ICP). We train a Triplet Network architecture to learn representations of the input data that can be used to estimate the similarity between test examples and examples in the training data set. Then, these representations are used to estimate the confidence of set predictions from a classifier that is based on the neural network architecture used in the triplet. The approach is evaluated using a robotic navigation benchmark and the results show that we can computed trusted confidence bounds efficiently in real-time.

==> introduction_old.tex <==
\section{Introduction}
%motivation, the benefits of using machine learning with cps
Machine learning components are being used by many cyber-physical system (CPS) applications because of their ability to generalize their training knowledge to handle dynamic and uncertain environments. One of the most common components is the Deep Neural Networks (DNN). Their advantage that makes them so attractive is their capacity to represent knowledge from large and multi-dimensional datasets as well as their ability to approximate complicated functions. 

%the problem, what are the challenges of usings DNNs with cps
The use of DNNs in safe critical systems such as CPS introduces many challenges that can have disastrous consequences if they don't get resolved. DNNs have been criticized by their inability to rationalize their predictions and are seen as black boxes. Modern DNN architectures are parameterized by over a million values that makes reviewing the decision process extremely hard. For this reason, they generally not provide well-calibrated confidence levels on their predictions. CPS on the other hand require operation under specifications and guarantees regarding the error rate. For DNNs to be able to provide error rate guarantees they need to be modified in a way so that their prediction will be coupled with an assurance measure.

%Other approaches to solve the problem, mention icp too
The popularity of the DNNs led to the development of different approaches that try to provide some kind of confidence estimation. Neural networks for classification typically provide probability-like outputs using a softmax layer. However, these probabilities are typically overconfident even for inputs coming from the same distribution as the training data~\cite{Guo:2017:CMN:3305381.3305518}. The reason is that the softmax probabilities are not well-calibrated, meaning they are not a good estimation of the actual probability distribution of the prediction.

There are different methods trying to produce calibrated probabilities for Neural Networks. There is a family of methods that estimates scaling factors from the training data and apply them to the softmax probabilities to improve their calibration. The most common of these methods is the temperature scaling~\cite{Guo:2017:CMN:3305381.3305518}. Other methods include Platt scaling \cite{Platt99probabilisticoutputs} and isotonic regression \cite{Zadrozny:2002:TCS:775047.775151}. Another framework developed to produce well-calibrated confidence values is conformal prediction~\cite{Vovk:2005:ALR:1062391,Shafer:2008:TCP:1390681.1390693,balasubramanian2014conformal} that uses calibration data to learn the accuracy of an underline model and estimates the models confidence based on how similar a test example is to the training data. DkNN is a method based on ICP that evaluates the similarity between data points by taking into account all the intermediate activation functions of a DNN~\cite{papernot2018deep}. A ML decision model is expected to perform better when a test example is similar to the used training data. A decision tree can be used split the training space to regions based on how data dense they are and assign prediction confidence measure to data coming from each region depending on the computed density~\cite{Gu:2019:TSM:3302509.3311038}.

%Our contribution, why triplet?
In our previous work~\cite{boursinos2020assurance}, we developed an assurance monitoring method based on the ICP framework. We designed a system architecture that work coupled with a DNN and can produce predictions with a predefined confidence bound. In order to achieve the chosen confidence our model may need to produce more than one possible decision. Sets with more than one predictions can be useful especially when the alternatives are given to a human operator. However we try to maximize the level of autonomy and compute the confidence bounds that are required in order for the model to generate single predictions.

This paper is an extension of our work on assurance monitors. The ICP framework requires the estimation of similarity between different samples. Since many applications make use of high-dimensional data, similarity tests between different samples are less accurate. For that reason we leverage the ability of Triplet networks to learn simple distance metrics, such us the euclidean distance, between any kind of data and investigate how this affect the performance of ICP.

%Organization
A formal definition of the problem follows in Section~\ref{sec:problem}. Sections \ref{sec:background} and \ref{sec:triplet} provide the background on ICP and Triplet respectively, that would be helpful for the reader to understand the operation of our derived system architecture. We evaluate the performance the suggested method using data from the SCITOS-G5 robot navigating around a room in Section~\ref{sec:evaluation} and compare it with a very similar architecture that does not utilize Triplet networks.

==> tables/execution_times.tex <==
\begin{table*}[ht]
% \fontsize{11}{13}\selectfont
\centering
\begin{tabular}{|c|c|c|c|}
\hline
NC Functions     & Memory Requirements & Triplet Execution Time & FC DNN Execution Time \\ \hline
$k$-NN           & 1.02 MB             & 1.4ms                  & 1.6ms                 \\ \hline
1-NN             & 3.5 MB              & 2.8ms                  & 3ms                   \\ \hline
Nearest Centroid & 180 kB              & 1.1ms                  & 1.4ms                 \\ \hline
\end{tabular}
\caption{Execution Times and Memory Requirements}
\label{tab:time_memory}
\end{table*}
